Balancing Lexicographic Fairness and a Utilitarian Objective with Application to Kidney Exchange

Balancing fairness and efficiency in resource allocation is a classical economic and computational problem. The price of fairness measures the worst-case loss of economic efficiency when using an inefficient but fair allocation rule; for indivisible goods in many settings, this price is unacceptably high. One such setting is kidney exchange, where needy patients swap willing but incompatible kidney donors. In this work, we close an open problem regarding the theoretical price of fairness in modern kidney exchanges. We then propose a general hybrid fairness rule that balances a strict lexicographic preference ordering over classes of agents, and a utilitarian objective that maximizes economic efficiency. We develop a utility function for this rule that favors disadvantaged groups lexicographically; but if cost to overall efficiency becomes too high, it switches to a utilitarian objective. This rule has only one parameter which is proportional to a bound on the price of fairness, and can be adjusted by policymakers. We apply this rule to real data from a large kidney exchange and show that our hybrid rule produces more reliable outcomes than other fairness rules.

==> fig_efficient_chains.tex <==
\begin{tikzpicture}[scale=1.0,transform shape]

\tikzstyle{graycirc}=[circle,draw=black,fill=lightgray,thin,inner sep=1.5pt,minimum size=8mm]
\tikzstyle{whitecirc}=[circle,draw=black,fill=white,thin,inner sep=1.5pt,minimum size=8mm]
\tikzstyle{blackcirc}=[circle,draw=black,fill=black,thin,inner sep=1.5pt,minimum size=8mm]
\tikzstyle{whitesq}=[rectangle,draw=black,fill=white,thin,inner sep=1.5pt,minimum size=5mm]

\node (bab) at (2,0) [whitecirc] {\tiny{B-AB}};
\node (ob) at (8,0) [whitecirc] {\tiny{O-B}};
\node (b) at (0,1) [whitesq] {\tiny{B}};
\node (abb) at (0,-1) [graycirc] {\tiny{AB-B}};
\node (o) at (4,-2) [whitesq] {\tiny{O}};
\node (abo) at (6,-2) [graycirc] {\tiny{AB-O}};
\node (bo) at (10,-2) [graycirc] {\tiny{B-O}};
\node (aab) at (2,-4) [whitecirc] {\tiny{A-AB}};
\node (oa) at (8,-4) [whitecirc] {\tiny{O-A}};
\node (ab) at (10,-4) [blackcirc] {\color{white}\tiny{A-B}};
\node (ba) at (12,-4) [blackcirc] {\color{white}\tiny{B-A}};
\node (aba) at (0,-3) [graycirc] {\tiny{AB-A}};
\node (a) at (0,-5) [whitesq] {\tiny{A}};
\node (ao) at (8,-2) [graycirc] {\tiny{A-O}};

\draw [latex-latex] (aba.east) -- (aab.north west);
\draw [-latex,dashed] (a.east) -- (aab.south west);
\draw [latex-latex] (abb.east) -- (bab.south west);
\draw [-latex,dashed] (b.east) -- (bab.north west);

\draw [-latex,dashed] (o.north east) -- (ob.north west);
\draw [-latex,dashed] (ob.north west) -- (bab.north east);

\draw [-latex,dashed] (abo.north) -- (ob.south west);
\draw [-latex,dashed] (ob.south west) -- (bab.south east);
\draw [-latex,dashed] (bab.south east) -- (abo.north);

\draw [-latex,dashed] (o.south east) -- (oa.south west);
\draw [-latex,dashed] (oa.south west) -- (aab.south east);

\draw [-latex,dashed] (abo.south) -- (oa.north west);
\draw [-latex,dashed] (oa.north west) -- (aab.north east);
\draw [-latex,dashed] (aab.north east) -- (abo.south);

\draw [latex-latex] (ao.south) -- (oa.north);

\draw [latex-latex] (bo.north west) -- (ob.south east);

\draw [-latex] (ab.north west) -- (bo.south west);
\draw [-latex] (bo.south west) -- (oa.north east);
\draw [-latex] (oa.north east) -- (ab.north west);

\draw [latex-latex] (ab.east) -- (ba.west);






\end{tikzpicture}

